Neuro-Symbolic AI in 2024: A Systematic Review

Background: The field of Artificial Intelligence has undergone cyclical periods of growth and decline, known as AI summers and winters. Currently, we are in the third AI summer, characterized by significant advancements and commercialization, particularly in the integration of Symbolic AI and Sub-Symbolic AI, leading to the emergence of Neuro-Symbolic AI. Methods: The review followed the PRISMA methodology, utilizing databases such as IEEE Explore, Google Scholar, arXiv, ACM, and SpringerLink. The inclusion criteria targeted peer-reviewed papers published between 2020 and 2024. Papers were screened for relevance to Neuro-Symbolic AI, with further inclusion based on the availability of associated codebases to ensure reproducibility. Results: From an initial pool of 1,428 papers, 167 met the inclusion criteria and were analyzed in detail. The majority of research efforts are concentrated in the areas of learning and inference (63%), logic and reasoning (35%), and knowledge representation (44%). Explainability and trustworthiness are less represented (28%), with Meta-Cognition being the least explored area (5%). The review identifies significant interdisciplinary opportunities, particularly in integrating explainability and trustworthiness with other research areas. Conclusion: Neuro-Symbolic AI research has seen rapid growth since 2020, with concentrated efforts in learning and inference. Significant gaps remain in explainability, trustworthiness, and Meta-Cognition. Addressing these gaps through interdisciplinary research will be crucial for advancing the field towards more intelligent, reliable, and context-aware AI systems.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> old_references.tex <==

% @InProceedings{Baran2022,
%   author    = {Baran, Joanna and Kocoń, Jan},
%   booktitle = {2022 IEEE International Conference on Data Mining Workshops (ICDMW)},
%   title     = {Linguistic Knowledge Application to Neuro-Symbolic Transformers in Sentiment Analysis},
%   year      = {2022},
%   month     = nov,
%   pages     = {395--402},
%   doi       = {10.1109/ICDMW58026.2022.00059},
%   issn      = {2375-9259},
%   keywords  = {Training;Knowledge engineering;Sentiment analysis;Conferences;Neural networks;Focusing;Linguistics;neuro-symbolic;sentiment analysis;WordNet;linguistic knowledge},
%   url       = {https://github.com/ExtensityAI/symbolicai},
% }

% @Article{Bu2021a,
%   author     = {Bu, Lei and Liang, Yongjuan and Xie, Zhunyi and Qian, Hong and Hu, Yi-Qi and Yu, Yang and Chen, Xin and Li, Xuandong},
%   journal    = {Form. Asp. Comput.},
%   title      = {Machine learning steered symbolic execution framework for complex software code},
%   year       = {2021},
%   issn       = {0934-5043},
%   month      = jun,
%   number     = {3},
%   pages      = {301--323},
%   volume     = {33},
%   address    = {Berlin, Heidelberg},
%   doi        = {10.1007/s00165-021-00538-3},
%   issue_date = {Jun 2021},
%   keywords   = {Symbolic execution, Machine learning, Nonlinear path condition, Constraint solving},
%   numpages   = {23},
%   publisher  = {Springer-Verlag},
%   url        = {https://github.com/ExtensityAI/symbolicai},
% }


% @article{Sen2021,
%  author = {Prithviraj Sen and Breno W. S. R. Carvalho and Ibrahim Abdelaziz and Pavan Kapanipathi and Francois Luus and Salim Roukos and Alexander Gray},
%  doi = {10.1109/csci54926.2021.00040},
%  journal = {arXiv preprint arXiv:2109.09566},
%  note = {Submitted 16 September, 2021; originally announced September 2021},
%  title = {Combining Rules and Embeddings via Neuro-Symbolic AI for Knowledge Base Completion},
%  url = {https://github.com/ExtensityAI/symbolicai},
%  year = {2021}
% }

